What Makes for Robust Multi-Modal Models in the Face of Missing Modalities?

With the growing success of multi-modal learning, research on the robustness of multi-modal models, especially when facing situations with missing modalities, is receiving increased attention. Nevertheless, previous studies in this domain exhibit certain limitations, as they often lack theoretical insights or their methodologies are tied to specific network architectures or modalities. We model the scenarios of multi-modal models encountering missing modalities from an information-theoretic perspective and illustrate that the performance ceiling in such scenarios can be approached by efficiently utilizing the information inherent in non-missing modalities. In practice, there are two key aspects: (1) The encoder should be able to extract sufficiently good features from the non-missing modality; (2) The extracted features should be robust enough not to be influenced by noise during the fusion process across modalities. To this end, we introduce Uni-Modal Ensemble with Missing Modality Adaptation (UME-MMA). UME-MMA employs uni-modal pre-trained weights for the multi-modal model to enhance feature extraction and utilizes missing modality data augmentation techniques to better adapt to situations with missing modalities. Apart from that, UME-MMA, built on a late-fusion learning framework, allows for the plug-and-play use of various encoders, making it suitable for a wide range of modalities and enabling seamless integration of large-scale pre-trained encoders to further enhance performance. And we demonstrate UME-MMA's effectiveness in audio-visual datasets~(e.g., AV-MNIST, Kinetics-Sound, AVE) and vision-language datasets~(e.g., MM-IMDB, UPMC Food101).

==> old_sections/old_sec4_experiments.tex <==
\section{Experiments}
\label{experiments}

In this section, we first attempt to quantify the modality complementarity of synthetic datasets using the proposed pipeline, and then employ that to help better comprehend real-world datasets in Sec~\ref{sec4.1_quantify}. 
In Sec~\ref{sec4.2_improving}, we demonstrate the effectiveness of proposed UME-Missing under missing-modality testing on  AV-MNIST~\cite{DBLP:journals/corr/abs-1808-07275}, Kinetics-Sound~\cite{DBLP:journals/corr/ArandjelovicZ17}, and AVE~\cite{DBLP:journals/corr/abs-2104-02000}.
Due to space constraints, we place the details about models and real-world datasets in Appendix \ref{sup3_details}.

\begin{figure}
\centering
\includegraphics[width=0.95\linewidth]{Image/twinx.pdf}
\caption{Estimated modality complementarity and model performance under missing-modality setting on the synthetic datasets and the Additive AV-MNIST dataset. When testing the model, we set different modalities to the missing mode, one at a time. The reported performance is the average of model accuracy in two missing-modality settings divided by the model accuracy in the complete-modality setting.
}
\label{fig:synthetic}
\vspace{-0.4cm}
\end{figure}

\subsection{Quantifying modality complementarity}
\label{sec4.1_quantify}
If the modalities are more complementary, the upper bound of the model performance in missing-modality testing will be lower. This problem cannot be resolved by designing more advanced methods, as the fundamental issue lies in the absence of information.
In this section, we first quantify the modality complementarity of synthetic datasets to demonstrate the effectiveness of our proposed pipeline. Further, we try to measure the modality complementarity of real-world datasets, which greatly enhances our understanding of multi-modal datasets.

\subsubsection{Synthetic dataset}
Inspired by prior research~\citep{DBLP:journals/corr/abs-2010-06572,DBLP:journals/corr/abs-2106-04538}, we first evaluate our pipeline on a well-designed synthetic dataset, which allows us to control the degree of modality complementarity. 
% Inspired by previous work~\citep{DBLP:journals/corr/abs-2010-06572} and~\citep{DBLP:journals/corr/abs-2106-04538}, we generate a set of synthetic data $(x,z,y)$. 
First, we sample random projection $P_X \in \mathbb{R}^{d_1\times d}$, $P_Z \in \mathbb{R}^{d_2\times d}$, and $P\in \mathbb{R}^{d\times d}$ from a uniform distribution $U(-0.5,0.5)$. Then we repeat following steps:\footnote{We sample 5000 data points with 80/20 train/val split and $\langle d,d_1,d_2,\delta \rangle=\langle 50,200,100,0.25\rangle$.}
\begin{enumerate}%[\hspace{0.5cm}Step 1.]
    \item Sample $x,z\in \mathbb{R}^d\sim \mathcal{N}(0,1)$.
    \item Set $z \gets (1-\alpha) z + \alpha x$; Then do projection $z\gets Pz$.
    \item Normalize $x,z$ to unit length; if $|x\cdot z|\leq \delta$, return to the Step 2.
    \item Generate the label $y$: If $x\cdot z > 0$, then $y=1$; else $y=0$. Return the tuple $(P_Xx, P_Zz, y)$.
\end{enumerate}
The $\alpha$ used in data generation controls the overlap between the two modalities $X,Z$. 
When $\alpha=0$, the modalities are independent and totally complementary in predicting the label $Y$. 
As $\alpha$ increases, their complementarity also decreases. 

We used several values of $\alpha$ to generate a series of synthetic datasets. 
For each of these datasets, we estimate the modality complementarity and evaluate the model's performance in missing-modality testing.
As shown in the left sub-figure of Figure~\ref{fig:synthetic}, as $\alpha$ increases, 
the modality complementarity we estimate decreases, which aligns well with the change in the complementarity of these datasets.
And the model is more capable of making accurate predictions under missing-modality testing because of the significant reduction in the complementary part of the modalities.
The results demonstrate the effectiveness of our pipeline for estimating modality complementarity and also support our analysis in Sec~\ref{sec3_1:preliminaries} and~\ref{sec3_2:bound}. In Appendix \ref{sup2_estimate}, we provide additional related results, such as the trend of each term in the formula for modality complementarity.
% The modality complementarity we estimate decreases, which verifies the effectiveness of our pipeline. 
% The trend of each term in the formula of modality complementarity can be found in the supplementary material.
% The results of estimated modality complementarity and model performance under missing-modality settings align well with our previous analysis. 

\subsubsection{Additive AV-MNIST}
To further evaluate our pipeline, we design a dataset named Additive AV-MNIST (AAV-MNIST), which is adapted from the AV-MNIST dataset~\citep{DBLP:journals/corr/abs-1808-07275}. The modality complementarity can be controlled by a parameter $\sigma$ in the data generation process. Below, we show how to generate AAV-MNIST dataset from the original AV-MNIST dataset, which has two modalities, image and audio, with labels ranging from 0 to 9. The following steps are repeated for every image $i$ in AV-MNIST:
\begin{enumerate}%[\hspace{0.5cm}Step 1.]
\item Let $x$ be the label of $i$. Sample $\delta \in \mathbb{R}\sim \mathcal{N}(0,\sigma)$ and round $\delta$ to the nearest integer. 
\item Set $y \gets (x+\delta) \mod 10$. Uniformly sample a spectrogram $s$ from all spectrograms in AV-MNIST with label $y$.
\item Calculate the new label $t \gets (x+y)/2$. Round $t$ to the nearest integer. Return the tuple $(i, s, t)$.
\end{enumerate}
When $\sigma$ is smaller, the image is more likely to indicate the same digit as its paired audio. This makes it easier to infer the label through a single modality, implying a lower level of modality complementarity.
In the right sub-figure of Figure~\ref{fig:synthetic}, the horizontal axis represents negative $\sigma$. 
As $\sigma$ approaches zero, the complementarity of multimodal data decreases. 
Correspondingly, the modality complementarity we estimate also declines. 
The model's performance in missing-modality testing improves as modality complementarity decreases, which also aligns with our previous analysis. The trend of each term in the formula for modality complementarity is also provided in Appendix \ref{sup2_estimate}.






\begin{figure}[t]
\begin{minipage}[b]{0.5\linewidth}
\centering
\captionof{table}{Our estimated modality complementarity on Additive AV-MNIST, Kinetics-Sounds and Hateful-Meme.}
\begin{tabular}{cc}
  \toprule
  Dataset & Est. Com. \\
        \midrule
                AAV-MNIST($\sigma=2.0$) &  0.9212\\
                Hateful-Meme~\citep{DBLP:journals/corr/abs-2005-04790} & 0.2403\\
                % AV-MNIST & 0.0490&  99.11& 56.06&10.00\\
			Kinetics-Sounds~\citep{DBLP:journals/corr/ArandjelovicZ17} & 0.0455\\
                % AVE & 0.0126 &78.61 & 39.80 &4.73\\
  \bottomrule
\end{tabular}
\label{tab:metric}
\end{minipage}
\hspace{0.5cm}
\begin{minipage}[t]{0.5\linewidth}
\centering
\includegraphics[width=\linewidth]{Image/hateful_meme.png}
\caption{Data examples from Hateful-Meme. The text is overlaid on the image for illustrative purposes, with the data sourced from ~\cite{DBLP:journals/corr/abs-2005-04790}. 
% As the examples demonstrate, it is necessary to fully observe both the image and the text to ascertain whether the data conveys any hateful meaning.
}
\label{fig:hateful}
\end{minipage} 
\vspace{-0.6cm}
\end{figure}






% The AAV-MNIST dataset is an extension of AV-MNIST dataset. 

% When $\sigma=0$, AAV-MNIST dataset is equivalent to AV-MNIST dataset where each image and its paired spectrogram represent the same number. 
% As $\sigma$ increases, each image become less correlated with its paired spectrogram, so they become more complementary for predicting the label $t$. 
% When $\sigma$ becomes very large, they are almost uncorrelated and the complementarity reaches the maximum. 

% We show in the plot \ref{fig:plots} that our metric reflects the complementarity of the AAV-MNIST dataset with different $\sigma$, indicating that our pipeline is effective in more complex settings beyond the synthetic dataset. Further, the robustness in the three settings verifies our conclusion that with other conditions unchanged, the more complementary the modalities are, the less robust the best model will be.

\subsubsection{Real-world datasets}
\label{sec4_1_3:real-world}
In this subsection, we further apply the pipeline for measuring modality complementarity to other real-world datasets: Hateful-Meme~\cite{DBLP:journals/corr/abs-2005-04790} and Kinetics-Sound~\cite{DBLP:journals/corr/ArandjelovicZ17}. The results are shown in Table~\ref{tab:metric}.
We have already known from Section 4.2 that the data in AAV-MNIST($\sigma=2.0$) is highly complementary due to its special design. 
But why is the complementarity of Hateful-Meme significantly higher than that of Kinetics-Sounds?

We include two examples of Hateful-Meme in Figure~\ref{fig:hateful} from \cite{DBLP:journals/corr/abs-2005-04790}.
We can see that two different images carry the same text, "Look how many people love you."
However, the right sub-figure features many people, while the left one doesn't contain any people.
Therefore, when the text is paired with the right sub-figure, they convey a positive meaning, but when paired with the left sub-figure, they carry a mean intention.
Hence, we can conclude that the different modalities in Hateful Memes are fairly complementary in predicting reasonable labels.
On the contrary, in Kinetics-Sound, the RGB modality can achieve strong performance individually~\cite{peng2022balanced}, indeed implying a lower level of modality complementarity. Thus, our proposed pipeline for estimating modality complementarity can indeed help us understand real-world datasets.
Further analyses of real-world datasets are included in Appendix \ref{sup2_estimate}. %\Li{Should we add a ref to the appendix page whenever we mention the supplementary material?}
%and also discuss the limitations of our current method for estimating modality complementarity.







\subsection{Improving model performance under missing-modality settings}
\label{sec4.2_improving}
In this subsection, we compare the performance of our proposed UME-Missing with several other methods under the missing-modality settings on AVE~\cite{DBLP:journals/corr/abs-2104-02000}, Kinetics-Sound~\cite{DBLP:journals/corr/ArandjelovicZ17}, and AV-MNIST~\cite{DBLP:journals/corr/abs-1808-07275}, which are all multi-modal datasets containing both audio and RGB modalities. Due to space limitations, we place more details about the datasets in Appendix~\ref{sup3_datasets}.

\textbf{Baseline Methods.}
The baseline methods compared include: 
(1) \emph{Naive Baseline}, which means end-to-end multi-modal learning from scratch without carefully designed tricks. We leverage the late fusion model, which is widely used in multi-modal learning~\cite{DBLP:journals/corr/abs-2104-02000}.
(2) \emph{Multi-task Training}. This method adds extra uni-modal linear classifiers to process the uni-modal features, which generates additional losses through the uni-modal outputs and the labels to jointly optimize the encoders. \cite{ma2022multimodal} use this technique to boost their model performance on missing-modality settings.
(3) \emph{Missing Augmentation}. This method randomly drops a modality in the input space and replaces it with constant noise, simulating the scenario of modality missing in actual situations. It is also compared in~\cite{ma2022multimodal}. 
(4) \emph{Missing Detection}. Inspired by out-of-distribution (OOD) detection~\cite{Vernekar2019OutofdistributionDI}, we assign a new category for the constant noise. 
During inference, if a uni-modal head predicts that a certain modality is missing, we rely on the prediction from the remaining modality. 
Otherwise, we ensemble the results from both modalities. We provide more explanation and details about these methods in Appendix~\ref{sup3_baselines}.
We also provides more experimental details about UME-Missing in Appendix~\ref{sup3_ume}.

\textbf{Results.}
We present the results of our UME-Missing and other methods under the missing-modality settings in Table~\ref{tab:ume_missing} (Note that all modalities are available during training, while one modality is missing during testing).
UME-Missing achieves the best results in most missing-modality cases.
Although for the missing-image case on the AV-MNIST dataset, the performance of UME-Missing is not the best, it is comparable with the best.
Furthermore, under normal multi-modal settings, the comparable performance of UME-Missing also demonstrates its advantage.































% \texttt{testtesttesttesttesttest}
% testtesttesttesttesttest
% \textnormal{testtesttesttesttesttest}
% \textcolor{gray}{testtesttesttesttesttest}
% We conduct experiments to verify the validity of our analysis and the effectiveness of our pipeline.
% We first introduce the training and testing settings and then show the results on the synthetic dataset, Additive AV-MNIST dataset, and real-world datasets. Unless otherwise specified, the missing/noise/adversarial robustness mentioned in the following subsections refers to the average accuracy under two sources of missing/noise/adversarial attack, divided by the model accuracy in the clean setting. For more detailed settings and results, please see Appendix \ref{sup2_details}. 
% \Li{Add introductions for each dataset here?}

% \textbf{Model Selection.} For the pre-trained feature extractors, we use Resnet18~\citep{DBLP:journals/corr/HeZRS15} and AudioNet (1-D CNN)~\citep{DBLP:journals/corr/abs-2104-02000} for Kinetics-Sounds and AVE, LeNet5~\citep{lecun1998gradient} and an 2-D CNN for AAV-MNIST, and Resnet152~\citep{DBLP:journals/corr/HeZRS15} and BERT~\citep{DBLP:conf/naacl/DevlinCLT19} for Hateful-Meme dataset. For the models tested for robustness, we use late fusion models for AVE, Kinetics-Sounds, and AV-MNIST, and we apply MMBT~\citep{DBLP:journals/corr/abs-1909-02950} for Hateful-Meme dataset.

% \textbf{Test setting.} For the missing image or audio, we substitute their value with zeros. For the missing text, we use a blank sentence $<$SOS$><$EOS$>$ as the input. 

% \textbf{Methods.} The baselines refer to direct training without any adjustment, the multi-task loss is the method used in previous work~\cite{ma2022multimodal}, the input augmentation means randomly dropping a modality during training with a fixed probability ($0.15$ for both modalities in AV-MNIST, $0.3$ for audio in Kinetics-Sounds, $0.1$ for video in Kinetics-Sounds, $0.25$ for both modality in AVE), and pretraining+finetuning means performing input augmentation on fixed pretrained networks for both modalities.

\begin{table}[t]
    \centering
    \caption{Top-1 test accuracy of UME-Missing and other methods under missing-modality settings and the normal setting. We also include the results of uni-modal models in the table as a reference. 
    Note that the performance of uni-modal models reflects the corresponding uni-modal model's performance using the available modality, whether audio or image. 
    For results that are used merely as a reference, we've rendered them in grey to distinguish them from the main results.
    }
    \vspace{5pt}

    \begin{tabular}{c|c|cc|c}
    \toprule
      Datasets   & Methods & Missing Image & Missing Audio & \textcolor{gray}{Multi-modal}\\
      \hline
      \multirow{6}{*}{AVE~\citep{DBLP:journals/corr/abs-2104-02000}}
    &\textcolor{gray}{Uni-Modal Models} & \textcolor{gray}{35.16\small{ $\pm$ 0.44}} & \textcolor{gray}{73.30\small{ $\pm$ 0.46}} & \textcolor{gray}{/}\\
    & Naive Baseline & 13.1\small{ $\pm$ 0.58} & 63.10\small{ $\pm$ 2.82} & \textcolor{gray}{77.45\small{ $\pm$ 0.22}} \\
    & Multi-task Training~\citep{ma2022multimodal} & 13.60\small{ $\pm$ 0.08} &58.29\small{ $\pm$ 0.08}  & \textcolor{gray}{76.94\small{ $\pm$ 0.44}} \\
    & Missing Augmentation & 23.80\small{ $\pm$ 0.17} & 66.25\small{ $\pm$ 0.08} & \textcolor{gray}{70.56\small{ $\pm$ 0.54}} \\
    & Missing Detection & 23.80\small{ $\pm$ 0.17} & 66.25\small{ $\pm$ 0.08} & \textcolor{gray}{70.56\small{ $\pm$ 0.54}} \\
    & \textbf{UME-Missing~(ours)} & \textbf{35.65\small{ $\pm$ 0.08}} & \textbf{72.47\small{ $\pm$ 0.08}} & \textcolor{gray}{80.02\small{ $\pm$ 0.22}}  \\
    \bottomrule
    
    \multirow{6}{*}{Kinetics-Sound~\citep{DBLP:journals/corr/ArandjelovicZ17}} & \textcolor{gray}{Uni-Modal Models} & \textcolor{gray}{26.57\small{ $\pm$ 0.08}} & \textcolor{gray}{62.57\small{ $\pm$ 0.09}} & \textcolor{gray}{/}\\
    & Naive Baseline & 17.08\small{ $\pm$ 0.16} & 57.52\small{ $\pm$ 0.15} & \textcolor{gray}{69.25\small{ $\pm$ 0.10}} \\
    & Multi-task Training~\citep{ma2022multimodal} & 21.98\small{ $\pm$ 0.14} & 58.02\small{ $\pm$ 0.15} & \textcolor{gray}{70.12\small{ $\pm$ 0.05}} \\
    
    & Missing Augmentation & 20.10\small{ $\pm$ 0.21} & 61.47\small{ $\pm$ 0.13} & \textcolor{gray}{67.04\small{ $\pm$ 0.11}} \\
    & Missing Detection & 20.90\small{ $\pm$ 0.28} & 62.35\small{ $\pm$ 0.02} & \textcolor{gray}{66.71\small{ $\pm$ 0.06}} \\
    & \textbf{UME-Missing~(ours)} & \textbf{25.34\small{ $\pm$ 0.04}} & \textbf{62.47\small{ $\pm$ 0.03}} & \textcolor{gray}{68.64\small{ $\pm$ 0.05}}  \\
    \bottomrule
    
      \multirow{6}{*}{AV-MNIST~\citep{DBLP:journals/corr/abs-1808-07275}} & \textcolor{gray}{Uni-Modal Models} & \textcolor{gray}{95.84\small{ $\pm$ 0.13}}   &\textcolor{gray}{97.29\small{ $\pm$ 0.02}} & \textcolor{gray}{/} \\ 
      % \cdashline{2-5}
      & Naive Baseline & 66.75\small{ $\pm$ 1.66} & 17.10\small{ $\pm$ 3.06} & \textcolor{gray}{99.10\small{ $\pm$ 0.03}}  \\
      % \cline{2-5}
      &Multi-task Training~\citep{ma2022multimodal} & 92.17\small{ $\pm$ 0.49} &  26.32\small{ $\pm$ 2.83} &\textcolor{gray}{99.51\small{ $\pm$ 0.18}}\\
      
      & Missing Augmentation & \textbf{95.16\small{ $\pm$ 0.08}} & 95.09\small{ $\pm$ 0.35} & \textcolor{gray}{99.65\small{ $\pm$ 0.09}}\\
    & Missing Detection & 94.45\small{ $\pm$ 0.32} & 95.99\small{ $\pm$ 0.21} &\textcolor{gray}{99.74\small{ $\pm$ 0.04}} \\    
    % \cdashline{2-5}
      & \textbf{UME-Missing~(ours)} & 94.32\small{ $\pm$ 0.05} & \textbf{97.27\small{ $\pm$ 0.02}} & \textcolor{gray}{99.53\small{ $\pm$ 0.02}}\\
  
    \bottomrule
    \end{tabular}
    \label{tab:ume_missing}
\end{table}
% missing detection & 70.56\small{ $\pm$ 0.54} & 66.25\small{ $\pm$ 0.08} & 23.80\small{ $\pm$ 0.17}\\
%                 pretraining+finetuning & 80.02\small{ $\pm$ 0.22} & 72.47\small{ $\pm$ 0.08} & 35.65\small{ $\pm$ 0.08} \\
% missing detection & 70.56\small{ $\pm$ 0.54} & 66.25\small{ $\pm$ 0.08} & 23.80\small{ $\pm$ 0.17}\\
% 76.94\small{ $\pm$ 0.44} & 58.29\small{ $\pm$ 0.08} & 13.60\small{ $\pm$ 0.08}
% \begin{table}[htbp]
%   \centering
%   \begin{tabular}{ccccc}
%   \toprule
%   Methods & multi-modal  & uni-image  & uni-audio  \\
%         \midrule
%                 multi-modal baseline &  99.10\small{ $\pm$ 0.03} & 17.10\small{ $\pm$ 3.06} &66.75\small{ $\pm$ 1.66}\\
%                 uni-image baseline & / & 97.29\small{ $\pm$ 0.02} & / \\
% 			uni-audio baseline & /&  /& 95.84\small{ $\pm$ 0.13} \\
% 			multi-task loss~\cite{ma2022multimodal} & 99.51\small{ $\pm$ 0.18} & 26.32\small{ $\pm$ 2.83} & 92.17\small{ $\pm$ 0.49}  \\
%                 missing detection & 99.81 & 96.14 & 94.04\\
%                 input augmentation & 99.65\small{ $\pm$ 0.09} & 95.09\small{ $\pm$ 0.35} & 95.16\small{ $\pm$ 0.08} \\
%                 pretraining+finetuning & 99.53\small{ $\pm$ 0.02} & 97.27\small{ $\pm$ 0.02} & 94.32\small{ $\pm$ 0.05} \\
%   \bottomrule
%   \end{tabular}
%   \caption{Evaluation on AV-MNIST~\cite{DBLP:journals/corr/abs-1808-07275}. The reported score is Accuracy(\%).}
%   \label{tab:avmnist}
% \vspace{-0.2cm}
% \end{table}
% \begin{table}[htbp]
%   \centering
%   \begin{tabular}{ccccc}
%   \toprule
%   Methods & multi-modal  & uni-image  & uni-audio  \\
%         \midrule
%                 multi-modal baseline &  69.49 & 57.75 &17.20\\
%                 uni-image baseline & / & 62.78 & / \\
% 				uni-audio baseline & /&  /& 25.89 \\
% 				multi-task loss~\cite{ma2022multimodal} & 70.04 & 58.06 & 21.03\\
%                 missing detection & 67.09 & 62.37 & 21.36\\
%                 input augmentation & 66.77 & 61.68 & 19.79 \\
%                 pretraining+finetuning & 68.40 & 62.50 & 25.69 \\
%   \bottomrule
%   \end{tabular}
%   \caption{Evaluation on Kinetics-Sounds~\cite{DBLP:journals/corr/ArandjelovicZ17}. The reported score is Accuracy(\%).}
%   \label{tab:ks}
% \vspace{-0.2cm}
% \end{table}
% \begin{table}[htbp]
%   \centering
%   \begin{tabular}{ccccc}
%   \toprule
%   Methods & multi-modal  & uni-image  & uni-audio  \\
%         \midrule
%                 multi-modal baseline &  77.45\small{ $\pm$ 0.22} & 63.10\small{ $\pm$ 2.82} &13.1\small{ $\pm$ 0.58}\\
%                 uni-image baseline & / & 73.30\small{ $\pm$ 0.46} & / \\
% 				uni-audio baseline & /&  /& 35.16\small{ $\pm$ 0.44} \\
% 				multi-task loss~\cite{ma2022multimodal} & 76.94\small{ $\pm$ 0.44} & 58.29\small{ $\pm$ 0.08} & 13.60\small{ $\pm$ 0.08}\\
%                 input augmentation & 72.55\small{ $\pm$ 0.29} & 64.51\small{ $\pm$ 0.33} & 26.20\small{ $\pm$ 0.42} \\
%                 missing detection & 70.56\small{ $\pm$ 0.54} & 66.25\small{ $\pm$ 0.08} & 23.80\small{ $\pm$ 0.17}\\
%                 pretraining+finetuning & 80.02\small{ $\pm$ 0.22} & 72.47\small{ $\pm$ 0.08} & 35.65\small{ $\pm$ 0.08} \\
%   \bottomrule
%   \end{tabular}
%   \caption{Evaluation on AVE~\cite{DBLP:journals/corr/abs-2104-02000}. The reported score is Accuracy(\%).}
%   \label{tab:ave}
% \vspace{-0.2cm}
% \end{table}



% \begin{figure}[t]
% \begin{minipage}[t]{\textwidth}
% \begin{minipage}[t]{0.5\textwidth}
% \makeatletter\def\@captype{table}
% \centering
% \caption{Evaluation on the encoders trained by naive multi-modal training and UMT.}
% \vspace{5pt}
% \begin{tabular}{c c c c c }
% 		\toprule
% 		\multirow{2}*{\textbf{Methods.}} & \multicolumn{2}{c}{\textbf{VGG-Sound}} & \multicolumn{2}{c}{\textbf{Kinetics-400}}\\
% 		\cline{2-5} & RGB & Audio & RGB & Audio\\
% 		\midrule
% 		Uni-Train & 23.2  & 45.2 & 74.1 & \textbf{23.5}\\
% 		MM Baseline & 15.9 &  18.3 & 72.9 & 18.3 \\
% 		UMT  & \textbf{24.4}  & \textbf{45.9} & \textbf{74.6} & 21.6\\
% 		\bottomrule
% \end{tabular}
% \label{tb:improve_encoders}
% \end{minipage}
% \begin{minipage}
% \begin{figure}
%     \centering
%     \includegraphics[width=0.4\linewidth]{Image/twinx.pdf}
%     \caption{Caption}
%     \label{fig:my_label}
% \end{figure}
% \end{minipage}
% % \begin{minipage}[t]{0.5\textwidth}
% % \makeatletter\def\@captype{table}
% % \centering
% % \caption{Self-Distillation vs UMT on VGG-Sound. }
% % \vspace{5pt}
% % \begin{tabular}{l|c}
% %     \toprule
% %     \textbf{Method}     & \textbf{Test Acc}      \\
% %     \midrule
% %     Baseline &   49.5     \\
% %     Self-Distill (label) & 49.7              \\
% %     Self-Distill (feature)  & 49.9           \\
% %     \midrule
% %     UMT & \textbf{53.5}\\
% %     \bottomrule
% % \end{tabular}
% % \label{tb:abla_distill}
% % \end{minipage}
% \end{minipage}
% \end{figure}

% \begin{figure}[ht]
% \begin{minipage}[b]{0.5\linewidth}
% \centering
% \captionof{table}{}
% \begin{tabular}{|c|c|}
% \hline
% Column 1 & Column 2\\
% \hline
% Value 1 & Value 2\\
% \hline
% \end{tabular}
% \label{tab:table1}
% \end{minipage}
% \hspace{0.5cm}
% \begin{minipage}[b]{0.5\linewidth}
% \centering
% \includegraphics[width=\linewidth]{Image/twinx.pdf}
% \caption{Example Image}
% \label{fig:image1}
% \end{minipage} 
% \end{figure}


==> old_sections/old_sec5_conclusions.tex <==
\section{Conclusions}
\label{conclusions}
% In this work, we partly explain the contradiction in previous conclusions on multi-modal robustness by pointing out the importance of the modality complementarity through information-theoretical analysis and carefully-designed experiments. As a reflection of modality interconnection, our proposed metric provides a basis for better understanding various multi-modal tasks and can be used beyond analyzing multi-modal robustness. 

In this work, we formally model the multi-modal data and define modality complementarity within the framework of information theory to better understand the intrinsic characteristics of multi-modal data and the performance of models under the missing-modality settings. 
We then propose a pipeline to empirically estimate the modality complementarity of multi-modal datasets. 
Furthermore, we introduce UME-Missing, which enhances the performance of models in the missing-modality settings.






==> old_sections/sup2_results.tex <==
\section{More experimental results}
In Sec~\ref{sec4.1_quantify}, we have quantified modality complementarity of various datasets. 
In this section, we first provide the trend of each term in the fromula for modality complementarity in synthetic datasets and Additive AV-MNIST as modality complementarity varies. 
And then we provide more additional results quantifying modality complementarity on other real-world datasets.
Finally, we also discuss scenarios of modality missing for datasets with high modality complementarity.

Please note, the choices of models and training details for the experiments are provided in Appendix~\ref{sup3_details}.




\label{sup2_results}
\subsection{More experimental results regarding quantifying modality complementarity}
\label{sup2_estimate}



\paragraph{The change of mutual information as modality complementarity varies.}

The change of each mutual information term in the calculation of our metric in synthetic datasets and AAV-MNIST is shown in the plots in Figure \ref{fig:supp_plots}. As the overlap of two modalities becomes larger, the amount of three mutual information terms grows with different rates. $I(X;Z)$ grows from nearly zero to large values, while $I(X;Y,Z)$ and $I(Z;Y,X)$ starts from non-zero values to larger values. The increasing amount of $I(X;Z)$ is larger than that of other two terms, leading to the decrease in our metric. The variance of mutual information terms is low except for the cases where $\alpha > 0.5$ in synthetic dataset. In the cases where $\alpha > 0.5$, the three mutual information terms all have large values and correspondingly high variance, resulting in the high variance of the metric which is close to zero. However, from our results of real-world datasets, we observed that the value of three terms are small and thus similar to the cases where $\alpha \leq 0.5$.  Hence, our metric is still indicative and effective for real-world datasets.
\begin{figure}
\centering
\includegraphics[width=1.0\linewidth]{Image/supp_mutualInfo.pdf}
\caption{Line plots showing the mean value of estimated mutual information terms with error bars (standard variances) on the synthetic dataset (left) and AAV-MNIST dataset (right). The mean values and standard variances are calculated from three independent repeated experiments. The x-axis is the parameter used in data generation. For synthetic dataset, we plot $\alpha$. For AAV-MNIST, we plot $-\sigma$ for unity. For synthetic data, $X$ refers to the modality with input dimension $=100$, and $Z$ refers to the modality with input dimension $=200$. For AAV-MNIST, $X$ refers to the audio, and $Z$ refers to the visual input.}
\label{fig:supp_plots}
\vspace{0.2cm}
\end{figure}
% \paragraph{Trend of each term in synthtic datasets.}

% \paragraph{Trend of each term in Additive AV-MNIST.}

% \subsection{Modality Complementarity on other real-world datasets.}

\paragraph{Modality Complementarity on more real-world datasets.}
The estimated modality complementarity on more real-world datasets is shown in Table \ref{tab:metric}. The low value in our metric of AVE, Kinetics-Sounds, and AV-MNIST indicates that they possess relatively little modality complementarity. In AV-MNIST, the two modalities reveal the heavy redundancy between their two modalities because each modality can give reasonable answers. And in AVE or Kinetics-Sound, the RGB modality can also give reasonable predictions individually, implying lower modality complementary. 
On the contrary, the modalities in the Hateful-Meme dataset are more complementary. This finding suits our intuition: In the Hateful-Meme dataset, altering the paired text of an image probably changes the label~\citep{kiela2020hateful}. Hence, only perceiving the image would not derive the right answer. 
% For the event classification task defined by Kinetics-Sounds and AVE, their audio and frames either lead to a rough answer. 

The model performance under missing-modality testing shown on the right demonstrates how modality complementarity affects model robustness. For comparison, we also provide the model performance in the clean setting (all modalities are complete) and the performance of a majority vote classifier, which always outputs the most common class in the training set and represents the lower bound of model performance. Note that we report the results of the model with the best performance for each dataset: For AV-MNIST, Kinetics-Sounds, and AVE, we use the UME-Missing, while for AAV-MNIST and Hateful-Meme, we use the Naive Baseline. Techniques that train models to perform better in missing-modality testing will fail in datasets with high modality complementarityz~(Please see the following section).
From the results, we observe that the missing case affects AAV-MNIST($\sigma=2.0$) and Hateful-Meme far more than the other three datasets: Their missing-modality performances are closer to the majority vote classifier. 
However, we also found cases where the estimates were not accurate. 
For instance, in AV-MNIST, any single modality can give very accurate predictions, but the estimated modality complementarity is higher than that of AVE or Kinetics-Sounds. This is primarily due to the fact that the process of calculating mutual information through MINE is an optimization process, and it may not be able to accurately compute the mutual information between different variables.






% Furthermore, the model robustness, especially the adversarial robustness, is also affected by factors other than modality complementarity. For instance, the model adversarial robustness of AVE and Kinetics-Sounds dataset is significantly lower than that of AV-MNIST dataset. We conjecture that this is related to the number of robust features in each modality of the datasets, which requires future work to confirm.

\begin{table}
  \centering
  \caption{Our estimated modality complementarity and tested model performance against missing modality on more real-world datasets. 
  We use Accuracy(\%) for AAV-MNIST, AV-MNIST, AVE and Kinetics-Sounds 
  and AUROC for Hateful-Meme (a binary classification task) as the evaluation score. 
  We also provide results in the clean setting and results of a majority vote classifier for reference. 
  For the "missing" column, we take the average accuracy of the model under the conditions of missing-image and missing-audio (or missing-text).
  In a majority vote classifier, the predicted class is always the most common class in the training set.}
  \begin{tabular}{ccccc}
  \toprule
  Dataset & Est. Complementarity & Clean & Missing &\textcolor{gray}{Majority}\\
        \midrule
                AAV-MNIST($\sigma=2.0$) &  0.9212& 64.35 &21.67&\textcolor{gray}{17.73}\\
                Hateful-Meme & 0.2403 & 70.36 & 53.45 &\textcolor{gray}{50.00}\\
                AV-MNIST & 0.0490&  99.53& 95.80&\textcolor{gray}{10.00}\\
				Kinetics-Sounds & 0.0455& 68.64  & 43.91 &\textcolor{gray}{3.14}\\
                AVE & 0.0126 &80.02 & 54.06 &\textcolor{gray}{4.73}\\
  \bottomrule
  \end{tabular}
  \label{tab:sup_metric}
% \vspace{-0.4cm}
\end{table}

\subsection{On missing modality in datasets with high modality complementarity}
\label{sup2_hm}

In Sec~\ref{sec4.2_improving}, we demonstrate that UME-Missing can significantly improve model performance in missing-modality testing on three datasets with relatively low modality complementarity. 
\emph{What about datasets with higher modality complementarity?}

Theoretically speaking, if modality complementarity is too high, a correct prediction would require the model to fully comprehend the relationships among different modalities. Without any one modality, the answers provided would lack a proper justification. 
This issue cannot be addressed by designing better algorithms, as it fundamentally results from the absence of information.

Empirically, we conducted relevant experiments on a real-world dataset with very high modality complementarity, specifically the Hateful Meme dataset. 
As shown in Table~\ref{tab:hm}, although UME-Missing indeed improved model performance in missing-modality testing, it is illogical to have a single modality provide a correct prediction during training. Or it could be said that it's a form of overfitting.
We hypothesize that this could harm the overall performance of the model. 
The poor performance of UME-Missing under multi-modal testing validates our assumption.


% \begin{table}[htbp]
%   \centering
%   \caption{Evaluation on Hateful-Meme~\cite{DBLP:journals/corr/abs-2005-04790}. The reported score is AUROC.}
%   \begin{tabular}{ccccc}
%   \toprule
%   Methods & multi-modal & uni-image & uni-text \\
%         \midrule
%                 multi-modal baseline & 68.63\small{ $\pm$ 0.91} & 49.45 &57.44\\
%                 uni-image baseline & / & 49.70\small{ $\pm$ 1.52} & / \\
% 				uni-text baseline & /&  /& 56.78\small{ $\pm$ 1.49} \\
%                 pretraining+finetuning & 59.69\small{ $\pm$ 1.38} & 54.83 & 60.19 \\
%   \bottomrule
%   \end{tabular}
%   \label{tab:hm}
% \end{table}


\begin{table}[htbp]
  \centering
  \caption{Evaluation on Hateful-Meme~\cite{DBLP:journals/corr/abs-2005-04790}. The reported score is AUROC.
  The meaning of each column can be referred to in Table~\ref{tab:ume_missing}.
  }
  \begin{tabular}{ccccc}
  \toprule
  Methods  & Missing Text & Missing Image & Multi-modal \\
    \midrule
    % \textcolor{gray}{Uni-modal Models} & \textcolor{gray}{49.70} & \textcolor{gray}{56.78} & \textcolor{gray}{/}\\
    Naive baseline & 49.45 &57.44 & \textbf{68.63}\\
    % uni-image baseline & / & 49.70\small{ $\pm$ 1.52} & / \\
    % uni-text baseline & /&  /& 56.78\small{ $\pm$ 1.49} \\
    \textbf{UME-Missing~(ours)} & \textbf{54.83} & \textbf{60.19} & 59.69\\
  \bottomrule
  \end{tabular}
  \label{tab:hm}
\end{table}


==> old_sections/sup3_details.tex <==
\section{Experiment details}
\label{sup3_details}
In this section, we provide detailed introductions about the real-world datasets we used, as well as thorough explanations of the models we used and training details supplementing Sec~\ref{sec3_3:quantifying},~\ref{sec4.1_quantify} and~\ref{sec4.2_improving}.


\subsection{Details of the estimation pipeline}
This sub-section provides additional details regarding Sec~\ref{sec3_3:quantifying} and ~\ref{sec4.1_quantify}.




\label{sup3_estimation}
\paragraph{Estimating pipeline.}
In Sec~\ref{sec3_3:quantifying}, we introduce the pipeline for estimating modality complementarity. To make this pipeline clearer, we visualize it in Figure~\ref{fig:structure}.
\begin{figure}
\centering
\includegraphics[width=1.0\linewidth]{Image/structure.pdf}
\caption{Pipeline to calculate the metric: First extract the features of the input data from two modalities by pre-trained models. Then apply the MINE to estimate the mutual information $I(Z;Y,X)$, $I(X;Y,Z)$, or $I(X;Z)$.}
\label{fig:structure}
% \vspace{-0.4cm}
\end{figure}

\paragraph{Details on estimating experiments.}
In Sec~\ref{sec4.1_quantify} and ~\ref{sup2_estimate}, we quantify the modality complementarity of different datasets. 
Details on Synthetic datasets and AAV-MNSIT are provided in Sec~\ref{sec4.1_quantify}.
Details on AVMNIST, Kinetics-Sounds, AVE and Hateful-Meme are provided in
Appendix ~\ref{sup3_datasets}.
Below, we supplement with the models used and training details for each dataset. 


\emph{1. Details on estimating modality complementarity of synthetic datasets.} The data generation method of synthetic data is described in section \ref{experiments}. Note that each class contains exactly half of all the data points. For the synthetic dataset, we do not employ feature extractors. We directly use the $200$-dim $X$ and $100$-dim $Z$ as the input for the estimators which are designed as following MLPs (See table \ref{tab:estimator_for_syn}). We use enough parameters to ensure the expressivity of the estimator. We train the estimators for 500 epochs and apply batch size $=100$. We use Adam as the optimizer, $10^{-3}$ as the learning rate, and $2\cdot 10^{-4}$ as the weight decay rate. 
\begin{table} [htbp]
  \centering
  \begin{tabular}{c|c}
  Layer & \# of Parameters \\
  \hline
  linear1 & $300\times 1000 + 1000$ \\
  \hline
  linear2 & $1000\times 500+500$\\
  \hline
  linear3 & $500\times 100+100$\\
  \hline
  linear4 & $100\times 1+1$
  \end{tabular}
  \begin{tabular}{c|c}
  Layer & \# of Parameters \\
  \hline
  linear1 & $300\times 1000 + 1000$\\
  \hline
  linear2 & $1000\times 200+200$\\
  \hline
  linear3 & $200\times 10+10$\\
  \hline
  linear4 & $12\times 12+12$\\
  \hline
  linear5 &$12\times 1+1$ 
  \end{tabular}
  \begin{tabular}{c|c}
  Layer & \# of Parameters \\
  \hline
  linear1 & $300\times 200 + 200$\\
  \hline
  linear2 & $200\times 2 + 2$
  \end{tabular}
  \caption{At left are the numbers of parameters in each layer for the estimator of $I(X;Z)$ for synthetic dataset. The activation function for linear1$\sim$3 is ELU and linear4 has no activation function. In the middle are the numbers of parameters in each layer for the estimator of $I(X;Z,Y)$ and $I(Z;X,Y)$ for synthetic dataset. The activation function for linear1$\sim$4 is ELU while linear5 has no activation function. The one-hot label is concatenated with the output of linear3 and then input to linear4. At right are the numbers of parameters in each layer of the trained two-layer perceptron for testing robustness.}
  \label{tab:estimator_for_syn}
\end{table}

\emph{2, Details on estimating modality complementarity of AAV-MNIST.} We employ pre-trained models for AAV-MNIST as feature extractors. Specifically, we first train a LeNet5~\citep{lecun1998gradient} for visual classification on AAV-MNIST and also a 2D-CNN for audio classification on AAV-MNIST. Then we use the output of the penultimate layer (before the final linear layer) as features, 84-dim for each modality. The estimator is designed as follows (See table \ref{tab:estimator_for_aav}).
\begin{table} [htbp]
  \centering
  \begin{tabular}{c|c}
  Layer & \# of Parameters \\
  \hline
  linear1 & $168\times 1000 + 1000$ \\
  \hline
  linear2 & $1000\times 100+100$\\
  \hline
  linear3 & $100\times 1+1$
  \end{tabular}
  \begin{tabular}{c|c}
  Layer & \# of Parameters \\
  \hline
  linear1 & $168\times 1000 + 1000$\\
  \hline
  linear2 & $1000\times 100+100$\\
  \hline
  linear3 & $110\times 110+110$\\
  \hline
  linear4 & $110\times 1+1$
  \end{tabular}
  \caption{At left are the numbers of parameters in each layer for the estimator of $I(X;Z)$ for AAV-MNIST dataset. The activation function for linear1$\sim$2 is ELU and linear3 has no activation function. At right are the numbers of parameters in each layer for the estimator of $I(X;Z,Y)$ and $I(Z;X,Y)$ for AAV-MNIST dataset. The activation function for linear1$\sim$3 is ELU while linear4 has no activation function. The one-hot label is concatenated with the output of linear2 and then input to linear3.}
  \label{tab:estimator_for_aav}
\end{table}

We train the estimators for 50 epochs and apply batch size $=800$. We set Adam as the optimizer, $10^{-3}$ as the learning rate for the first forty epochs and $10^{-4}$ for the last ten epochs, and $10^{-4}$ as the weight decay rate. 

\emph{3, Details on estimating modality complementarity of Kinetics-Sounds and AVE.} We train a Resnet18~\citep{DBLP:journals/corr/HeZRS15} for visual classification and AudioNet (1-D CNN)~\citep{DBLP:journals/corr/abs-2104-02000} for audio classification. Then we use the output of the penultimate layer (before the final linear layer) as features, 512-dim for each modality. The estimator is designed as follows (See table \ref{tab:estimator_for_real}).
\begin{table} [htbp]
  \centering
  \begin{tabular}{c|c}
  Layer & \# of Parameters \\
  \hline
  linear1 & $1024\times 1000 + 1000$ \\
  \hline
  linear2 & $1000\times 100+100$\\
  \hline
  linear3 & $100\times 1+1$
  \end{tabular}
  \begin{tabular}{c|c}
  Layer & \# of Parameters \\
  \hline
  linear1 & $1024\times 1000 + 1000$\\
  \hline
  linear2 & $1000\times 100+100$\\
  \hline
  linear3 & $128\times 128+128$\\
  \hline
  linear4 & $128\times 1+1$
  \end{tabular}
  \caption{At left are the numbers of parameters in each layer for the estimator of $I(X;Z)$ for AVE and Kinetics-Sounds dataset. The activation function for linear1$\sim$2 is ELU and linear3 has no activation function. At right are the numbers of parameters in each layer for the estimator of $I(X;Z,Y)$ and $I(Z;X,Y)$ for AVE dataset. For Kinetics-Sounds, linear3 has $127\times 127+127$ parameters and linear4 has $127\times 1+1$ parameters. The activation function for linear1$\sim$3 is ELU while linear4 has no activation function. The one-hot label is concatenated with the output of linear2 and then input to linear3.}
  \label{tab:estimator_for_real}
\end{table}

For AVE dataset, we train the estimators for 30 epochs and apply batch size $=96$. We use Adam as optimizer, $10^{-3}$ as learning rate and $10^{-4}$ as weight decay rate. For Kinetics-Sounds dataset, we train the estimators for 30 epochs and apply batch size $=384$. We use Adam as the optimizer, $10^{-2}, 10^{-3}, 10^{-4}$ as the learning rate for 0$\sim$10, 10$\sim$20, and 20$\sim$30 epochs, respectively. We set $10^{-5}$ as the weight decay rate. 

In practice, when estimating mutual information between $A$ and $B$, we found that when the correlation between $A$ and $B$ is small, a larger learning rate should be used. However, a too-large learning rate quickly leads to an explosion due to the exponential term. The batch size should also be relatively small to increase the update frequency. 

\emph{4, Details on estimating modality complementarity of Hateful-Meme.} We adopt the data processing and augmentation used in~\citep{mmfsingh2020}. We use a Resnet152~\citep{DBLP:journals/corr/HeZRS15} for visual input and BERT~\citep{DBLP:conf/naacl/DevlinCLT19} for texts. Then we extract the 2048-dimensional visual features and 768-dimensional language features, and use an estimator for calculating mutual information. The estimator is designed as follows (See table \ref{tab:estimator_for_hateful}).
\begin{table} [htbp]
  \centering
  \begin{tabular}{c|c}
  Layer & \# of Parameters \\
  \hline
  linear1 & $2816\times 1000 + 1000$ \\
  \hline
  linear2 & $1000\times 100+100$\\
  \hline
  linear3 & $100\times 1+1$
  \end{tabular}
  \begin{tabular}{c|c}
  Layer & \# of Parameters \\
  \hline
  linear1 & $2816\times 1000 + 1000$\\
  \hline
  linear2 & $1000\times 100+100$\\
  \hline
  linear3 & $102\times 102+102$\\
  \hline
  linear4 & $102\times 1+1$
  \end{tabular}
  \caption{At left are the numbers of parameters in each layer for the estimator of $I(X;Z)$ for Hateful-Meme dataset. The activation function for linear1$\sim$2 is ELU and linear3 has no activation function. At right are the numbers of parameters in each layer for the estimator of $I(X;Z,Y)$ and $I(Z;X,Y)$ for Hateful-Meme dataset. The activation function for linear1$\sim$3 is ELU while linear4 has no activation function. The one-hot label is concatenated with the output of linear2 and then input to linear3.}
  \label{tab:estimator_for_hateful}
\end{table}
For the Hateful-Meme dataset, we train the estimators for 30 epochs and apply batch size $=128$. We use AdamW as the optimizer, $10^{-2}$ as the learning rate and $10^{-8}$ as the epsilon. We train the estimators for 30 epochs and apply batch size $=128$. \Li{Todo.} We use AdamW as the optimizer, $10^{-2}$ as the learning rate and $10^{-8}$ as the epsilon. 

\subsection{Details of the models used to predict the labels.}
\label{sup3_testing}
\paragraph{Training details.}
The backbones of models used to predict the labels of the datasets are the same to those in estimating pipeline.
As for the fusion modules, all datasets used a linear fusion head to produce outputs~\cite{du2023uni}, except for Hateful Meme. The fusion module for Hateful Meme is MMBT~\cite{DBLP:journals/corr/abs-1909-02950}.

For \textbf{AVMNIST}, we use SGD as the optimizer, and the batch size and learning rate is 64 and 0.01, respectively. The total training epochs is 20.
For \textbf{AVE}, we use SGD as the optimizer, and the batch size is also 64. The learning rate of visual encoder and other parameters is 1e-4 and 1e-3, respectively. The total training epochs is 30. Every 10 epochs, we reduce the learning rate to one-tenth of its original value.
For \textbf{Kinetics-Sound}, we also use SGD as the optimizer, and the batch size is 256. 
The learning rate of visual encoder and other parameters is 1e-4 and 1e-3, respectively.
The total training epochs is 30. Every 10 epochs, we reduce the learning rate to one-tenth of its original value.
\paragraph{Missing-modality testing details.}
In the missing-modality testing, we fill in the missing modality with all zeros except the text of Hateful Meme. For the missing text in Hateful Meme, we use a blank sentence $<$SOS$><$EOS$>$ as the input. 



% \textbf{Synthetic dataset.} 
% For missing-modality performance testing, we trained a simple two-layer perceptron neural network. In the missing modality setting, we fill in the missing modality with zeros. 

% \textbf{AAV-MNIST.} We test the missing-modality performance of a late-fusion model for classification. It uses the pre-trained LeNet5 and 2D-CNN as feature extractors, concatenates their outputs, and uses a linear layer as the fusion layer. During training, the feature extractors and the fusion layer are trained jointly. In the missing modality setting, we fill in the missing modality with all zeros.

% \textbf{Real-world datasets.} For the missing image or audio, we substitute them with all zeros. For the missing text, we use a blank sentence $<$SOS$><$EOS$>$ as the input. 

\subsection{Details of real-world datasets}
\label{sup3_datasets}
\textbf{AV-MNIST and Additive AV-MNIST.} The AV-MNIST dataset~\cite{DBLP:journals/corr/abs-1808-07275} contains two modalities: Disturbed images and audio spectrograms. The image is from the $28\times 28$ PCA-projected MNIST images with $75\%$ energy removed. The $112\times 112$ audio spectrograms are the pronounced digits augmented with noise samples. The size of the AV-MNIST dataset is the same as that of the MNIST dataset (with train/test splits of 60000/10000). For the Additive AV-MNIST dataset (AAV-MNIST), the data generation method is also in section \ref{experiments}. So the size of the AAV-MNIST dataset is the same as that of the AV-MNIST dataset. To magnify the contrast between AAV-MNIST with different $\sigma$, we alter the energy-eliminating rate in the original AV-MNIST dataset by reducing it from $75\%$ to $25\%$. In this way, the image can be more indicative of the target $Y$. We do not use data augmentation for AAV-MNIST, except that the inputs are all scaled to the range $[-1, 1]$ (spectrogram) or $[0, 1]$ (image).

\textbf{AVE.} The AVE dataset~\cite{DBLP:journals/corr/abs-1803-08842} contains 4,143 unconstrained videos spanning 28 event categories including Rodents, Accordion, and Mandolin. It has the train/val splits of 3,339/402 videos. For AVE and Kinetics-Sounds, we adopt the data processing and augmentation used in~\cite{DBLP:journals/corr/abs-2104-02000}. Note that the inputs are all scaled to the range $[-1, 1]$ (spectrogram) or $[0, 1]$ (image).

\textbf{Kinetics-Sounds.} The Kinetics-Sounds dataset~\cite{DBLP:journals/corr/ArandjelovicZ17, DBLP:journals/corr/CarreiraZ17} consists of YouTube videos with manually
annotated human actions. It is a subset with 32 classes from Kinetics400, such as playing\_harmonica, tapping\_pen, and shoveling\_snow. It has the train/val splits of 22728/1592.

% 9309/3104/3103 \Li{Recount this number.}.

\textbf{Hateful-Meme.} The Hateful-Meme dataset defines the task of identifying hate speech in memes. It has two classes of image-text pairs: hateful and benign. The same image with different captions can have different labels, so this dataset is expected to have a high degree of modal complementarity. It has the train/val splits of 8500/500.

\subsection{Details of UME-Missing}
\label{sup3_ume}
In terms of the model's choice and training details, UME-Missing and the naive baseline are highly consistent.
Compared to the naive baseline, UME-Missing enhances the learning by employing uni-modal pre-trained backbones for the encoders and incorporating Missing-modality Augmentation.

\paragraph{Hyper-parameters for Missing-modality Augmentation.} For AVMNIST, we set the image to be in a missing state with a probability of 0.2, and similarly, the audio is in a missing state with a probability of 0.2.
For AVE, we set the image to be in a missing state with a probability of 0.25, and similarly, the audio is in a missing state with a probability of 0.25.
For Kinetics-Sound, we set the image to be in a missing state with a probability of 0.3, and similarly, the audio is in a missing state with a probability of 0.1.
Note that we never put both image and audio in a missing state at the same time, and all missing modalities are filled with zeros.



% \textbf{Model Selection.} 
% For the pre-trained feature extractors, we use Resnet18~\citep{DBLP:journals/corr/HeZRS15} and AudioNet (1-D CNN)~\citep{DBLP:journals/corr/abs-2104-02000} for Kinetics-Sounds and AVE, LeNet5~\citep{lecun1998gradient} and an 2-D CNN for AAV-MNIST, and Resnet152~\citep{DBLP:journals/corr/HeZRS15} and BERT~\citep{DBLP:conf/naacl/DevlinCLT19} for Hateful-Meme dataset. For the models tested for robustness, we use late fusion models for AVE, Kinetics-Sounds, and AV-MNIST, and we apply MMBT~\citep{DBLP:journals/corr/abs-1909-02950} for Hateful-Meme dataset.

\subsection{Details of baseline methods}
\label{sup3_baselines}
% \Li{In this section, we can additionally analyze why these methods do not work.}
Here we offer a more detailed introduction and analysis of the baseline methods we compare against.

\begin{itemize}
    \item \emph{Naive Baseline}, which means end-to-end multi-modal learning from scratch without carefully designed tricks. We leverage the late fusion model, which is widely used in multi-modal learning~\cite{DBLP:journals/corr/abs-2104-02000}. However, this method has not been specifically trained for missing-modality testing, so it generally performs poorly under missing-modality conditions.
    \item \emph{Multi-task Training}. This method adds extra uni-modal linear classifiers to process the uni-modal features, which generates additional losses through the uni-modal outputs and the labels to jointly optimize the encoders. \cite{ma2022multimodal} use this technique to boost their model performance on missing-modality settings. This method is designed to allow each encoder to train better. However, due to potential optimization issues caused by multiple losses~\cite{yu2020gradient}, the models trained with this method only achieve sub-optimal results.
    \item \emph{Missing Augmentation}. This method randomly drops a modality in the input space and replaces it with constant noise, simulating the scenario of modality missing in actual situations. It is also compared in~\cite{ma2022multimodal}. However, during training, the gradients of the encoder with the missing modality acts as noise, greatly affecting the training of the encoder with the missing modality. Therefore, the model's performance in testing is not satisfactory.
    \item \emph{Missing Detection}. Inspired by out-of-distribution (OOD) detection~\cite{Vernekar2019OutofdistributionDI}, we assign a new category for the constant noise. During inference, if a uni-modal head predicts that a certain modality is missing, we rely on the prediction from the remaining modality. Otherwise, we ensemble the results from both modalities. 
\end{itemize}

As shown in Table~\ref{tab:ume_missing}, overall, our method surpasses other methods, being both simple and effective.







==> old_sections/sup4_limitations.tex <==
% \section{Limitations}
% \label{sup4_limitations}
% \Li{Refine this part to fit the current content.}
% The first limitation of our work is that our computation of the proposed metric is an optimization process, which leads to a small computational overhead and a concern about error margin. 

% Second, our study does not reveal all factors of multi-modal robustness. In section \ref{experiments}, we suggest a possible factor, the number of robust features in each modality, which deserves further work to confirm. Other factors that affect the robustness of multi-modal models include the model architecture (e.g., CNN, ViT, and various fusion methods) and the training pipeline (e.g., pre-training, adversarial training), which are used to achieve better performance or robustness. Apart from architecture and pipeline, factors like the anti-noise ability of each modality also matter (e.g., maybe images are more robust against noise than audios). However, we could study their property using uni-modal settings and tools. This paper focuses on modal complementarity, which is brought by the interconnection of modalities. So it distinguishes multi-modal robustness study from uni-modal robustness study, and this is the reason why we pay so much attention to this factor.

% There are several possible directions for future work. First, to lower the estimation variance for our metric, the estimator can be improved by substituting MINE with more efficient and accurate estimators or adjusting the network architecture of the estimator.

% Second, other factors that affect multi-modal robustness can be pointed out and analyzed. For example, how do different fusions affect the multi-modal robustness, and what are their mechanisms? Can we distinguish the impacts of different factors on multi-modal robustness and diagnose the problem of a given vulnerable multi-modal model? How do we combine these factors to achieve maximal robustness?

% Finally, more fine-grained analysis on multi-modal attack and robustness can be conducted. For instance, do the adversarial attacks damage the complementary part more or the shared part more? Conversely, do the defense methods in uni-modal learning work for multi-modal learning, and which part do they benefit? Can we extract the robust features and non-robust features in multi-modal learning like what researchers have done in uni-modal learning? How do we improve the multi-modal robustness based on our knowledge of the interconnection of modalities (e.g. modal complementarity) of a specific task?

==> old_sections/sup5_extensions.tex <==
\section{Extensions}
\label{sup5_extensions}
In the main text, we primarily discuss how to measure modality complementarity in datasets with two modalities. It can be extended to more modalities.


\subsection{Modality Complementarity among More Than Two Modalities}
\label{sup5_morethantwo}
In this section, we discuss how to extend modaility complementarity to cases with more than two modalities. 
Denote the modalities as $S=\{X_1,X_2,\dots, X_m\}$. We can choose a subset $S_1\subset S$ and focus on the complementarity of $S_1$. So we are dividing all modalities into two parts. Denote $S_2 = S\setminus S_1$, and we have the following relation:
\begin{align*}
    I(S_1,S_2;Y) &= \Gamma_{S_1} + \Gamma_{S_2} + I(S_1;Y;S_2)
\end{align*}
We define the complementarity metric of $S_1$ as
\begin{align*}
    \frac{\Gamma_{S_1}}{I(S;Y)} &= \frac{I(S_1;Y | S_2)}{I(S;Y)}=\frac{I(S_1;Y,S_2) - I(S_1;S_2)}{I(S;Y)}
\end{align*}

We can calculate this metric using the pipeline in section \ref{sec3_3:quantifying}. We test our analysis on a synthetic dataset with $m$ modalities where we can adjust the degree of modality overlap by the parameter $\alpha$. Extending the settings in section \ref{sec4.1_quantify}, we generate a set of synthetic data $(\{x_i|i\in [m]\}, y)$ with $m=4$: First, sample random projection $P_i \in \mathbb{R}^{d_1\times d}$ and $Q_i\in \mathbb{R}^{d\times d}$, $\forall i\in [m]$ from a uniform distribution $U(-0.5,0.5)$. Then sample 10000 data points with 80/20 train/val split with the following steps:
\begin{enumerate}%[\hspace{0.5cm}Step 1.]
\item Sample $x_i\in \mathbb{R}^d\sim \mathcal{N}(0,1)$, $\forall i\in [m]$.
\item Set $x_i \gets (1-\alpha) x_i + \alpha x_1$ and then do projection $x_i\gets P_i x_i$, $\forall i\in [m]\setminus \{1\}$.
\item Normalize all $x_i$ to unit length, $\forall i\in [m]$.
\item If $|(x_1+x_2)\cdot (x_3+x_4)|\leq \delta$, return to the Step 2.
\item Generate the label $y$: If $(x_1+x_2)\cdot (x_3+x_4) > 0$, then $y=1$; else $y=0$. \item Return the tuple $(\{Q_ix_i \mid i\in [m]\}, y)$.
\end{enumerate}
We set $\langle d,d_1,\delta \rangle=\langle 50,50,0.25\rangle$.
We calculate the complementarity for $S_1=\{x_2\}$ and perform missing-modality testing on two-layer perceptron neural networks trained on the datasets with different $\alpha$: When $\alpha=0$, the modalities are complementary in predicting the label $Y$. When $\alpha=1$, they can give correct predictions individually. 
As $\alpha$ increases, the modality complementarity in this dataset decreases.

Similar to the settings for the synthetic dataset with two modalities, we do not employ feature extractors. We directly use the raw data as the input for the estimators designed as following MLPs (See table \ref{tab:estimator_for_syn4}). We train the estimators for $1000$ epochs and apply batch size $=1000$. Other hyperparameters are the same as in section \ref{sup3_estimation}.

The results are shown in Figure \ref{fig:plots_4modalities}, which shows that the estimated modality complementarity aligns with the designed property of the data.
% our pipeline can still estimate the proposed metric and quantify the complementarity of $S_1$. 
As the modality complementarity decreases, the model's performance on missing-modality testing also increases, supporting our theoretical results.
% Compared with datasets with two modalities, the impact of overlap degree on the robustness towards single source attack/corruption is lighter. 


\begin{figure}
\centering
\includegraphics[width=1.0\linewidth]{Image/Synthetic-4modalities.pdf}
\caption{At left is the line plot showing the mean value of the estimated modality complementarity (blue line) with error bars (standard variances) of three independent repeated experiments and the missing-modality performance of the models (orange line) on the synthetic dataset. 
The missing robustness refers to the accuracy where $x_2$ is missing, then divided by the clean accuracy. 
At right is the line plots showing the mean value of estimated mutual information terms with error bars (standard errors) where $X$ refers to the modality set $S_1=\{x_2\}$ and $Z$ refers to $S_2=\{x_1,x_3,x_4\}$.}
\label{fig:plots_4modalities}
\vspace{-0.4cm}
\end{figure}
\begin{table} [!htbp]
  \centering
  \begin{tabular}{c|c}
  Layer & \# of Parameters \\
  \hline
  linear1 & $200\times 1000 + 1000$ \\
  \hline
  linear2 & $1000\times 500+500$\\
  \hline
  linear3 & $500\times 100+100$\\
  \hline
  linear4 & $100\times 1+1$
  \end{tabular}
  \begin{tabular}{c|c}
  Layer & \# of Parameters \\
  \hline
  linear1 & $200\times 1000 + 1000$\\
  \hline
  linear2 & $1000\times 500+500$\\
  \hline
  linear3 & $500\times 100+100$\\
  \hline
  linear4 & $102\times 12+12$\\
  \hline
  linear5 &$12\times 1+1$ 
  \end{tabular}
  \begin{tabular}{c|c}
  Layer & \# of Parameters \\
  \hline
  linear1 & $200\times 200 + 200$\\
  \hline
  linear2 & $200\times 2 + 2$
  \end{tabular}
  \caption{At left are the parameters in each layer for the estimator of $I(X;Z)$ for the synthetic dataset. At the right are the parameters in each layer of the trained two-layer perceptron for testing robustness. Other settings, including the activation function type, are the same as in section \ref{sup3_estimation}.}
  \label{tab:estimator_for_syn4}
\end{table}
% \subsection{Applying the Metric}
% \label{sup5_application}
